MXene Fe2C as a promising candidate for the 2D XY ferromagnet

Monolayer Fe$_2$C is expected to possess strong electronic correlations, which can significantly contribute to electronic and magnetic properties. In this work we consider electronic and magnetic properties of MXene Fe$_2$C within the DFT+DMFT approach. We establish the existence of local magnetic moments $\mu=3.2\mu_B$ in this compound, characterized by sufficiently long lifetime of $\tau\sim 350$ fs. We also calculate exchange interaction parameters accounting for electronic correlations using the recently developed approach for paramagnetic phase. We obtain the strongest exchange interaction $11$ meV between next nearest neighboring Fe atoms above (and below) the carbon plane, and the subleading interaction $6$ meV between the next to next nearest neighboring atoms across the carbon plane. The resulting dependence of the Berzinskii-Kosterlitz-Thouless (BKT) and Curie temperatures on magnetic anisotropy is obtained. The BKT temperature for the pristine Fe$_2$C is $T_{\rm BKT}\simeq 290$ K, which makes this compound a good candidate for the two-dimensional ferromagnet with XY anisotropy.

==> preambule.tex <==
\usepackage{graphicx}
\usepackage{float}
\usepackage{hyperref}
\hypersetup{
    colorlinks=false,
    pdfborder={0 0 1},
    % linkcolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
    pdftitle={Overleaf Example},
    pdfpagemode=FullScreen,
}


